On Kernel's Safety in the Spectre Era (Extended Version)

The efficacy of address space layout randomization has been formally demonstrated in a shared-memory model by Abadi et al., contingent on specific assumptions about victim programs. However, modern operating systems, implementing layout randomization in the kernel, diverge from these assumptions and operate on a separate memory model with communication through system calls. In this work, we relax Abadi et al.'s language assumptions while demonstrating that layout randomization offers a comparable safety guarantee in a system with memory separation. However, in practice, speculative execution and side-channels are recognized threats to layout randomization. We show that kernel safety cannot be restored for attackers capable of using side-channels and speculative execution and introduce a new condition, that allows us to formally prove kernel safety in the Spectre era. Our research demonstrates that under this condition, the system remains safe without relying on layout randomization. We also demonstrate that our condition can be sensibly weakened, leading to enforcement mechanisms that can guarantee kernel safety for safe system calls in the Spectre era.

==> discussion.tex <==

% \paragraph*{Comparison with \Cref{Abadi}}
% % Before delving into the details of this result, we would like to compare our model with that of \Citet{Abadi} in order to show why their result cannot be directly applied to the scenario of kernel address space layout randomization, KASLR for short. 

% The execution model of~\Cref{sec:language} is based
% on that of \cite{Abadi,Abadi2,Abadi3} (in particular
% to that of \citet{Abadi3}), but it has undergone some
% substantial modifications because of the intention
% to study the effectiveness of KASLR as
% a protection measure for operating systems. To this aim,
% the language of our victims has been equipped with constructs for
% pointer arithmetic indirect jump and with different
% privilege execution modes that modify, at runtime,
% the accessible address-space.
% % These changes
% % are meant to make our model as close as possible to that
% % of a real world kernel: the code of a kernel is mostly
% % written low level language and it runs in a privileged
% % execution mode, while user-space programs ---
% % the attackers --- run in an unprivileged one, but can
% % temporarily change the execution mode by issuing a syscall.
% % Depending on the privilege level the running program can
% % access different memory areas, i.e. the victim and the
% % attacker have disjoint address spaces.

% These modifications are why, the results of \Citet{Abadi}
% cannot directly apply to our scenario:
% in that work, the goal of the attacker was to directly
% access private locations of the victim's memory.
% But this kind of attack cannot take place in our model by definition:
% here any memory access to a valid kernel-space address
% when the system is in \emph{user-mode} would fail because of
% the disjoint address spaces.
% This is why, in this work, the goal of the
% attacker is to take advantage of the interaction with the
% system calls in order to trigger one of these to access an
% allocated address that the victim system call is not meant to access.
% % We think that this threat model can capture a large class
% % of real world attacks; for instance, all those attacks which
% % are meant to trigger the kernel-space execution of
% % arbitrary code, or to write to arbitrary kernel
% % memory fall within this category. 

\paragraph*{\emph{Kernel Safety}, Memory Safety and CFI}
In this section, we discuss how the notion of \emph{kernel safety}
relates with other common safety properties. In particular, we want to show
that \emph{kernel safety} encompasses some
form of \emph{spatial memory safety} and of \emph{control flow integrity},
that are maybe the most sought-after properties in operating systems
security research, as witnessed by the large number of
measures that together with layout randomization have been proposed
for their enforcement~\cite{kCFI,RustInLinux,towardkernelsafety,HyperSafe,FineGrainedkCFI,CompProtKer}.

\emph{Spatial memory safety} can be stated in different
ways~\cite{PierceMS,HighAssurance,SoftBound,MSWasm}, but
all these definitions associate a software component
(a program, an instruction, or even a variable) with a fixed memory area,
that this component can access rightfully. A memory access outside
these bounds consists in a violation of \emph{spatial memory safety}.

It is easy to see that our notion of \emph{kernel safety} encompasses
a form of spatial memory safety: if a system enjoys \emph{kernel safety},
then no system call can access a memory that does not appear within its \tcaps.
In particular, every system call $\syscall$ can only access
arrays that are mentioned within $\caps(\syscall)$.

% In general, \emph{spatial memory safety} is not a robust property~\cite{MSWasm};
% and \emph{a fortiori}, it is not true that any probabilistic weakening of
% spatial memory safety is also robust with respect to unprivileged attackers.

% However, \Cref{thm:scenario2}, precisely states that \emph{speculative kernel safety}
% is robust with respect to user-space attackers. Similarly, from \Cref{thm:scenario1},
% we dedeuce that  our syscalls are memory safe if taken individually (\Cref{lemma:onsyspms}),
% \emph{and} that they enjoy \emph{kernel safety} even when linked to an arbitrary attacker.
% However, this property fails when the system is extended with new syscalls. For instance,
% we can take the following system:
% %
% \begin{align*}
%   \syscall () &\defsym \ret \ass \aone & \caps(\syscall)&\defsym \{\aone\}\\
%   \syscalltwo (\vx) &\defsym \cmemread \vy \vx  & \caps(\syscall)&\defsym \{\}
% \end{align*}
% %
% In this example, \Cref{lemma:onsyspms} ensures that  both the syscalls are
% individually memory safe up to a certain probability. However, as witnessed by
% the user-space program $\csyscall \syscall {}\sep \csyscall\syscalltwo\ret$,
% memory safety is broken with probability 1 when the system is linked with
% an arbitrary user-space program. Similarly, if we take a system where every
% syscall is \emph{speculative kernel safe}, and we add a syscall which does not
% enjoy this property, then it is trivial to see that the resulting system
% does not enjoy\emph{speculative kernel safe}. To sum up:
% \emph{(speculative) kernel safety} are robust with respect to
% unprivileged attackers and are not robust with respect to extension of the system
% with possibly unsafe code.

\emph{Kernel safety} also provides some form of control flow integrity guarantees~\cite{CFI}.
This property requires that the indirect jumps and returns operation
performed by a program can reach only specific targets that usually
can be statically determined. % Here, we are interested in discussing which form of
% \emph{control flow integrity} is provided by \emph{kernel safety}.
%
% In the literature, different flavors of control flow integrity have been studied:
% in particular, we talk about \emph{forward-edge} CFI, when the integrity of the target
% is granted only on indirect jumps, and we talk about \emph{backward-edge} CFI when
% it refers to return addresses.

Our semantics prevents the execution of a function
if its address fors not belong to the set of \tcaps
of the current system call. This means that if a system
$\system = (\rfs, \syss, \caps)$ is
\emph{kernel safe}, then every system call $\syscall$ enjoys a form
of \emph{forward-edge} CFI with respect to the completely connected
graphs whose nodes are all the elements of $\caps(\syscall)\cap \Funk$.

% Due to the choice of not modeling activation records' stacks,
% \emph{kernel safety} does not offer any guarantee of \emph{backward-edge}
% control flow integrity. We believe adding a stack of activation records in memory
% to our model and studying kernel safety in that context is interesting open
% question that we leave to future work. 

% \paragraph*{Enforcement of \emph{Speculative Kernel Safety}}
% Finally, we would like to comment on our approach to the enforcement of
% \emph{speculative kernel safety}. In \Cref{sec:sksenforcement}, we found that
% that property can be enforced on any \emph{kernel safe} system by applying
% a language-level transformation on the system that makes vulnerabilities
% \emph{classically backed}. As an example, we showed the fencing
% transformation, but the reader may argue that in practice,
% the time-overhead of a similar mitigation would be unfavorable.
% However, \Cref{lemma:onsystrans} shows that any system transformation that
% turns a system into an equivalent system with classically backed vulnerabilities
% makes \emph{kernel safe} systems \emph{speculative kernel safe}.
% In particular, this means that, the transformation may also make use
% of other more sophisticated mechanisms such as formal verification,
% language based mechanisms or compiler-based solutions to reduce the number of fences
% and thus the performance overhead. Moreover, while the fencing transformation is
% somehow specific to our model, the requirements of \Cref{lemma:onsystrans}
% are general and can be applied to a large variety of execution models.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper.tex"
%%% End:

==> rules1arxiv.tex <==
\begin{figure*}[h!]
  \small
  \centering
  \columnwidth=\linewidth
  \begin{framed}
    \[
      \Infer[WLE][Load]
      { \step
        {\ntc{\cmemread \vx \expr\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {\ntc{\cmd}{\update{\regmap}{x}{\mem(\add)}}{\opt}{\st}{\mem}}
      }
      {
        \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
        % \mem(\add) \in \Val &
        \add \in \underline \lay(\Ar[\opt]) &
        \fbox{$\opt = \km[\syscall] \Rightarrow \add \in \underline \lay(\caps(\syscall))$}
      }
    \]
    
    \resizebox{\textwidth}{!}{\(
      \Infer[WLE][Load-Error]
      {\step
        {\ntc{\cmemread \vx \expr\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
        {\err }
      }
      {
        \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
        \add \not\in \underline \lay(\Ar[\opt])
      }
      \quad
      \Infer[WLE][Load-Unsafe]
      {\step
        {\ntc{\cmemread \vx \expr\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
        {\unsafe}
      }
      {
        \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
        \add \in \underline \lay(\Ar[\km]) &
        \fbox{$\add \not\in \underline \lay(\caps(\syscall))$}
      }
      \)}\\[0mm]
    %
    \[
      \Infer[WL][Store]
      { \step
        {\ntc{\cmemass \expr \exprtwo\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {\ntc{\cmd}{\regmap}{\opt}{\st}{\update{\mem}{\add}{\sem \exprtwo_{\regmap, \lay}}}}
      }
      {
        \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
        % \mem(\add) \in \Val &
        \add \in \underline \lay(\Ar[\opt]) &
        \fbox{$\opt = \km[\syscall] \Rightarrow \add \in \underline \lay(\caps(\syscall))$}
      }
    \]
    \[
      \Infer[WL][Store-Error]
      {\step
        {\ntc{\cmemass \expr \exprtwo\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {\err}
      }
      {\toAdd{\sem\expr_{\regmap, \lay}} = \add &
        \add \notin \underline \lay(\Ar[\opt])
      }
      \quad
      \Infer[WL][Store-Unsafe]
      {\step
        {\ntc{\cmemass \expr \exprtwo\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
        {\unsafe}
      }
      {
        \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
        \add \in \underline \lay(\Ar[\km]) &
        \fbox{$\add \not\in \underline \lay(\caps(\syscall))$}
      }
    \]\\[0mm]
    %
    \resizebox{\textwidth}{!}{\(
      \Infer[WLE][Call]{
        \step
        {\ntc{\ccall{\expr}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {
          \ntc
          {\mem(\add)}
          {\regmap_0[\vx_{1} \upd \sem{\exprtwo_1}_{\regmap,\lay}, \dots, \vx_{n} \upd \sem{\exprtwo_n}_{\regmap,\lay}]}
          {\opt}
          {\frame{\cmd}{\regmap}{\opt} : \st}
          {\mem}
        }
      }
      {\toAdd{\sem{\expr}_{\regmap, \lay}}=\add &
        \add \in \underline \lay(\Fn[\opt]) &
        \fbox{$\opt = \km[\syscall] \Rightarrow \add \in \underline \lay(\caps(\syscall))$}
      }
      \)}

    \[
      \Infer[WLE][Call-Error]{
        \step
        {\ntc{\ccall{\expr}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {\err}
      }
      {
        \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
        \add \not\in \underline \lay(\Fn[\km])
      }
    \]
    
    \[
      \Infer[WLE][Call-Unsafe]{
        \step
        {\ntc{\ccall{\expr}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
        {\unsafe}
      }
      {
        \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
        \add \in \underline \lay(\Fn[\km]) &
        \fbox{$\add \not\in \underline \lay(\caps(\syscall))$}
      }
    \]\\[0.5mm]
    %
    \resizebox{\textwidth}{!}{\(
      \Infer[WLE][SystemCall][\textsc{SC}]{
        \step
        {\ntc{\csyscall{\syscall}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {
          \ntc
          {\syss(\syscall)}
          {\regmap_0[\vx_{1} \upd \sem{\exprtwo_1}_{\regmap,\lay}, \dots, \vx_{n} \upd \sem{\exprtwo_n}_{\regmap,\lay}]}
          {\km[\syscall]}
          {\frame{\cmd}{\regmap}{\opt} : \st}
          {\mem}
        }
      }
      {
        \phantom{~}
      }
      \)}\\[0.5mm]
    %
    \[
      \Infer[WLE][Pop]{
        \step
        {\ntc{\cnil}{\regmap}{\opt}{\frame {\cmd} {\regmap'} {\opt'}\cons \st}{\mem}}
        {\ntc{\cmd}{\update{\regmap'}{\ret} {\regmap(\ret)}}{\opt'}{\st}{\mem}}
      }
      {}
    \]

    \[
      \Infer[WLE][Skip]
      { \step
        {\ntc{\cskip\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {\ntc{\cmd}{\regmap}{\opt}{\st}{\mem}}
      }
      {
      }
    \]

    \[
      \Infer[WLE][Op]
      { \step
        {\ntc{\vx \ass \expr\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
        {\ntc{\cmd}{\update{\regmap}{\vx}{\sem \expr_{\regmap, \lay}}}{\opt}{\st}{\mem}}
      }
      {
      }
    \]

    \[
      \Infer[WLE][If]
      { \step
        {\ntc{\cif \expr {\cmd_\ctrue} {\cmd_\cfalse}\sep\cmdtwo}{\regmap}{\opt}{\st}{\mem}}
        {\ntc{\cmd_{\toBool{\sem \expr_{\regmap, \lay}}}\sep \cmdtwo}{\regmap}{\opt}{\st}{\mem}}
      }
      {
      }
    \]  

    \[
      \Infer[WLE][While]
      { \step
        {\ntc{\cwhile {\expr} {\cmd}\sep\cmdtwo}{\regmap}{\opt}{\st}{\mem}}
        {\confone_{\toBool{\sem \expr_{\regmap, \lay}}}}
      }
      {
        \confone_{\ctrue} = {\ntc{\cmd\sep\cwhile {\expr} {\cmd}\sep \cmdtwo}{\regmap}{\opt}{\st}{\mem}} &
        \confone_{\cfalse} = {\ntc{\cmdtwo}{\regmap}{\opt}{\st}{\mem}}     }
    \]
  \end{framed}
  \caption{Semantics w.r.t. system $\system=(\rfs,\syss,\caps)$.}
  \label{fig:stepexcerpt}
\end{figure*}

% \begin{figure*}[h!]
%   \centering
%   \columnwidth=\linewidth
%   \begin{framed}
%   \[
%     \Infer[WLE][Load]
%     { \step
%         {\ntc{\cmemread \vx \expr\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%         {\ntc{\cmd}{\update{\regmap}{x}{\mem(\add)}}{\opt}{\st}{\mem}}
%     }
%     {
%       \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
%       % \mem(\add) \in \Val &
%       \add \in \underline \lay(\Ar[\opt]) &
%       \fbox{$\opt = \km[\syscall] \Rightarrow \add \in \underline \lay(\caps(\syscall))$}
%     }
%   \]

%   \[
% \Infer[WLE][Load-Error]
%     {\step
%         {\ntc{\cmemread \vx \expr\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
%         {\err }
%     }
%     {
%       \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
%       \add \not\in \underline \lay(\Ar[\opt])
%     }
%     \quad
%     \Infer[WLE][Load-Unsafe]
%     {\step
%         {\ntc{\cmemread \vx \expr\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
%         {\unsafe}
%     }
%     {
%       \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
%       \add \in \underline \lay(\Ar[\km]) &
%       \fbox{$\add \not\in \underline \lay(\caps(\syscall))$}
%     }
%   \]

%     \[
%       \Infer[WL][Store]
%       { \step
%         {\ntc{\cmemass \expr \exprtwo\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%         {\ntc{\cmd}{\regmap}{\opt}{\st}{\update{\mem}{\add}{\sem \exprtwo_{\regmap, \lay}}}}
%       }
%       {
%         \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
%         % \mem(\add) \in \Val &
%         \add \in \underline \lay(\Ar[\opt]) &
%         \fbox{$\opt = \km[\syscall] \Rightarrow \add \in \underline \lay(\caps(\syscall))$}
%       }
%     \]
    
%     \[
%       \Infer[WL][Store-Error]
%       {\step
%         {\ntc{\cmemass \expr \exprtwo\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%         {\err}
%       }
%       {\toAdd{\sem\expr_{\regmap, \lay}} = \add &
%         \add \notin \underline \lay(\Ar[\opt])
%       }
%       \quad
%       \Infer[WL][Store-Unsafe]
%       {\step
%         {\ntc{\cmemass \expr \exprtwo\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
%         {\unsafe}
%       }
%       {
%         \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
%         \add \in \underline \lay(\Ar[\km]) &
%         \fbox{$\add \not\in \underline \lay(\caps(\syscall))$}
%       }
%     \]
  
%   \[
%     \Infer[WLE][Call]{
%       \step
%       {\ntc{\ccall{\expr}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%       {
%         \ntc
%          {\mem(\add)}
%          {\regmap_0[\vx_{1} \upd \sem{\exprtwo_1}_{\regmap,\lay}, \dots, \vx_{n} \upd \sem{\exprtwo_n}_{\regmap,\lay}]}
%          {\opt}
%          {\frame{\cmd}{\regmap}{\opt} : \st}
%          {\mem}
%       }
%     }
%     {\toAdd{\sem{\expr}_{\regmap, \lay}}=\add &
%       \add \in \underline \lay(\Fn[\opt]) &
%       \fbox{$\opt = \km[\syscall] \Rightarrow \add \in \underline \lay(\caps(\syscall))$}
%     }
%   \]

%   \[
%     \Infer[WLE][Call-Error]{
%       \step
%         {\ntc{\ccall{\expr}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%         {\err}
%     }
%     {
%       \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
%       \add \not\in \underline \lay(\Fn[\km])
%     }
%     \quad
%     \Infer[WLE][Call-Unsafe]{
%       \step
%         {\ntc{\ccall{\expr}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\km[\syscall]}{\st}{\mem}}
%         {\unsafe}
%     }
%     {
%       \toAdd{\sem{\expr}_{\regmap, \lay}} = \add &
%       \add \in \underline \lay(\Fn[\km]) &
%       \fbox{$\add \not\in \underline \lay(\caps(\syscall))$}
%     }
%   \]

%   \[
%     \Infer[WLE][SystemCall]{
%       \step
%       {\ntc{\csyscall{\syscall}{\exprtwo_1,\dots,\exprtwo_n}\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%       {
%         \ntc
%          {\syss(\syscall)}
%          {\regmap_0[\vx_{1} \upd \sem{\exprtwo_1}_{\regmap,\lay}, \dots, \vx_{n} \upd \sem{\exprtwo_n}_{\regmap,\lay}]}
%          {\km[\syscall]}
%          {\frame{\cmd}{\regmap}{\opt} : \st}
%          {\mem}
%       }
%     }
%     {
%     }
%   \]
  
%   \[
%     \Infer[WLE][Pop]{
%       \step
%       {\ntc{\cnil}{\regmap}{\opt}{\frame {\cmd} {\regmap'} {\opt'}\cons \st}{\mem}}
%       {\ntc{\cmd}{\update{\regmap'}{\ret} {\regmap(\ret)}}{\opt'}{\st}{\mem}}
%     }
%     {}
%   \]

%     \[
%     \Infer[WLE][Skip]
%     { \step
%         {\ntc{\cskip\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%         {\ntc{\cmd}{\regmap}{\opt}{\st}{\mem}}
%     }
%     {
%     }
%     \quad
%     \Infer[WLE][Op]
%     { \step
%         {\ntc{\vx \ass \expr\sep\cmd}{\regmap}{\opt}{\st}{\mem}}
%         {\ntc{\cmd}{\update{\regmap}{\vx}{\sem \expr_{\regmap, \lay}}}{\opt}{\st}{\mem}}
%     }
%     {
%     }
%   \]

%   \[
%     \Infer[WLE][If]
%     { \step
%         {\ntc{\cif \expr {\cmd_\ctrue} {\cmd_\cfalse}\sep\cmdtwo}{\regmap}{\opt}{\st}{\mem}}
%         {\ntc{\cmd_{\toBool{\sem \expr_{\regmap, \lay}}}\sep \cmdtwo}{\regmap}{\opt}{\st}{\mem}}
%     }
%     {
%     }
%   \]  

%   \[
%     \Infer[WLE][While]
%     { \step
%         {\ntc{\cwhile {\expr} {\cmd}\sep\cmdtwo}{\regmap}{\opt}{\st}{\mem}}
%         {\confone_{\toBool{\sem \expr_{\regmap, \lay}}}}
%     }
%     {
%       \confone_{\ctrue} = {\ntc{\cmd\sep\cwhile {\expr} {\cmd}\sep \cmdtwo}{\regmap}{\opt}{\st}{\mem}} &
%       \confone_{\cfalse} = {\ntc{\cmdtwo}{\regmap}{\opt}{\st}{\mem}}     }
%   \]
%   \end{framed}
%   \caption{Semantics w.r.t. system $\system=(\rfs,\syss,\caps)$, excerpt of the rules.}
%   \label{fig:stepexcerpt}
% \end{figure*}

